Tool-Policy Co-Design for Powder Weighing in Laboratory Automation

Autonomous powder weighing is one of many bottlenecks in laboratory automation due to the complex, non-linear dynamics of heterogeneous materials. Robot chemists performing this task utilise standard tools shaped for the dexterity of human hands, whose fixed geometry sets the dynamics that the control policy needs to regulate. This work introduces a tool-policy co-design framework that concurrently optimises the morphology of a dispensing tool and its control policy for use by robots in chemistry laboratories, formulated as a bi-level optimisation that minimises dispensing error over a target distribution of powder flowabilities. The outer loop varies tool-design parameters such as tool depth, width and rim spike topology using Bayesian optimisation and hyperband, while an inner loop optimises a control policy for each candidate morphology. We also introduce a geometric similarity metric that warm-starts policy training from cached policies of structurally similar designs, exploring 28% more configurations under the same compute budget. The proposed framework is evaluated on a robotic powder weighing task across seven materials with distinct physical dynamics in a flowability-informed robot-material simulation framework. Experimental results demonstrate that our co-designed tool morphology reduces real-world weighing errors by 45% relative to a standard tool, including on previously unseen materials. These results demonstrate our method can adapt both the control policy and the physical tool to the dynamics of the target material, bringing a new paradigm for material manipulation to the field of laboratory automation.

==> tables/bohb_vs_bohb.tex <==
\begin{table}[h]
    \caption{Simulation and real life deployment comparison of the standard BOHB optimiser and the one using Similarity filtering}
    \centering
    \resizebox{0.99\linewidth}{!}{% % Resizes to 95% of the column width
        \begin{NiceTabular}{l *{8}{c}}[hlines, cell-space-limits=3pt]
            \hline % Using a single hline at the very top
            \Block{2-1}{Optimisation Method} & \multicolumn{3}{c}{\textbf{Spoon Configuration}} & \Block{2-1}{Simulation Steps} &\Block{2-1}{Simulation Error}  & \Block{2-1}{Real life Error } \\
            % Removed the cmidrule here
             & Depth & Width & Spike Configuration & & \\
             \hline
            \midrule % Keeping midrule for separation before the data rows
            BOHB &\\
            Similarity BOHB  & \\
            \bottomrule % Keeping bottomrule at the very end
        \end{NiceTabular}
    }
\end{table}
